NASH: Neural Architecture and Accelerator Search for Multiplication-Reduced Hybrid Models

The significant computational cost of multiplications hinders the deployment of deep neural networks (DNNs) on edge devices. While multiplication-free models offer enhanced hardware efficiency, they typically sacrifice accuracy. As a solution, multiplication-reduced hybrid models have emerged to combine the benefits of both approaches. Particularly, prior works, i.e., NASA and NASA-F, leverage Neural Architecture Search (NAS) to construct such hybrid models, enhancing hardware efficiency while maintaining accuracy. However, they either entail costly retraining or encounter gradient conflicts, limiting both search efficiency and accuracy. Additionally, they overlook the acceleration opportunity introduced by accelerator search, yielding sub-optimal hardware performance. To overcome these limitations, we propose NASH, a Neural architecture and Accelerator Search framework for multiplication-reduced Hybrid models. Specifically, as for NAS, we propose a tailored zero-shot metric to pre-identify promising hybrid models before training, enhancing search efficiency while alleviating gradient conflicts. Regarding accelerator search, we innovatively introduce coarse-to-fine search to streamline the search process. Furthermore, we seamlessly integrate these two levels of searches to unveil NASH, obtaining the optimal model and accelerator pairing. Experiments validate our effectiveness, e.g., when compared with the state-of-the-art multiplication-based system, we can achieve $\uparrow$$2.14\times$ throughput and $\uparrow$$2.01\times$ FPS with $\uparrow$$0.25\%$ accuracy on CIFAR-100, and $\uparrow$$1.40\times$ throughput and $\uparrow$$1.19\times$ FPS with $\uparrow$$0.56\%$ accuracy on Tiny-ImageNet. Codes are available at \url{https://github.com/xuyang527/NASH.}

==> Tables/alg-cifar.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\setlength{\tabcolsep}{3.5pt}
\caption{Comparisons between ours and SOTA multiplication-based/-free/-reduced baselines in terms of operation numbers, \huihong{computational energy costs (\texttt{Comp.})}, and accuracy (\texttt{Acc.}), when tested on CIFAR10 and CIFAR100.} 
\renewcommand{\arraystretch}{1.1}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|ccccc|ccccc}
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{\textbf{Models}}                                           & \multirow{2}{*}{\textbf{Methods}}  & \multicolumn{5}{c|}{\textbf{CIFAR10}}                                                                 & \multicolumn{5}{c}{\textbf{CIFAR100}}                                                                \\ \cline{3-12} 
                                                                           &                                                                                                                             & \textbf{Multi. (M)} & \textbf{Shift (M)} & \textbf{Add (M)} & \textbf{Comp. (mJ)} & \textbf{Acc. (\%)} & \textbf{Multi. (M)} & \textbf{Shift (M)} & \textbf{Add (M)} & \textbf{Comp. (mJ)} & \textbf{Acc. (\%)} \\ \hline \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Multi.-\\ Based\end{tabular}}   & AlphaNet                                                                                                                      & 72.86              & 0.00               & 72.86            & 0.437               & 95.86             & 76.02              & 0.00               & 76.02            & 0.456               & 79.10             \\
                                                                           & PreNAS-A                                                                                                               & 85.46              & 0.00               & 85.46            & 0.513               & 96.09             & 94.82              & 0.00               & 94.82            & 0.569               & 79.61             \\
                                                                           & PreNAS-B                                                                                                              & 69.85              & 0.00               & 69.85            & 0.419               & 95.90             & 75.90              & 0.00               & 75.90            & 0.455               & 79.40             \\
                                                                           & PreNAS-C                                                                                                              & 60.37              & 0.00               & 60.37            & 0.362               & 95.72             & 64.92              & 0.00               & 64.92            & 0.390               & 78.98             \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Multi.-\\ Free\end{tabular}}    & DeepShift-MV2 \cite{DeepShift}                                                                                                           & 6.60               & 79.20              & 85.80            & 0.154               & 91.90             & 6.70               & 79.20              & 85.80            & 0.154               & 71.00             \\
                                                                           & AdderNet-MV2 \cite{AdderNet}                                                                                                           & 6.60               & 0.00               & 165.00           & 0.154               & 89.50             & 6.70               & 0.00               & 165.00           & 0.154               & 63.50             \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Multi.-\\ Reduced\end{tabular}} & NASA-F-A                                                                                                                   & 50.87              & 28.53              & 85.42            & 0.351               & 95.96             & 72.48              & 15.68              & 107.34           & 0.471               & 79.68             \\
& NASA-F-B                                                                                                                   & 46.78              & 43.88              & 103.60           & 0.353               & 95.87             & 59.72              & 14.84              & 88.26            & 0.390               & 79.42             \\
& NASA-F-C                                                                                                                   & 41.90              & 40.84              & 94.02            & 0.318               & 95.72             & 53.26              & 18.82              & 87.70            & 0.358               & 79.17             \\
                                                                           & \rowcolor{dark-green!15}\textbf{Ours-A}                                                                                                           & \textbf{55.48}     & \textbf{33.81}     & \textbf{95.76}   & \textbf{0.386}      & \textbf{96.16}    & \textbf{71.04}     & \textbf{19.04}     & \textbf{112.02}  & \textbf{0.469}      & \textbf{80.09}   \\
                                                                           & \rowcolor{dark-green!15}\textbf{Ours-B}                                                                                                           & \textbf{47.97}     & \textbf{33.81}     & \textbf{88.24}   & \textbf{0.341}      & \textbf{96.06}    & \textbf{65.97}     & \textbf{18.64}     & \textbf{105.78}  & \textbf{0.438}      & \textbf{79.85}   \\
                                                                           & \rowcolor{dark-green!15}\textbf{Ours-C}                                                                                                          & \textbf{42.26}     & \textbf{33.13}     & \textbf{81.85}   & \textbf{0.306}      & \textbf{95.87}    & \textbf{56.61}     & \textbf{14.14}     & \textbf{88.52}   & \textbf{0.373}      & \textbf{79.63}   \\ \Xhline{3\arrayrulewidth}
\end{tabular}} \label{tab:alg-exp-cifar} 
\end{table*}

==> Tables/alg-tiny.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\setlength{\tabcolsep}{4pt}
\caption{Comparisons of operation numbers, \huihong{computational energy costs (\texttt{Comp.})}, and accuracy (\texttt{Acc.}) between ours and the most competitive baseline AlphaNet \cite{AlphaNet} on Tiny-ImageNet.} 
\renewcommand{\arraystretch}{1.1}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|ccccc}
\Xhline{3\arrayrulewidth}
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Models}}}                               & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Methods}}} & \multicolumn{5}{c}{\textbf{Tiny-ImageNet}}                                                                                                                           \\ \cline{3-7} 
\multicolumn{1}{c|}{}                                                      & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c}{\textbf{Multi. (M)}} & \multicolumn{1}{c}{\textbf{Shift (M)}} & \multicolumn{1}{c}{\textbf{Add (M)}} & \multicolumn{1}{c}{\textbf{Comp. (mJ)}} & \multicolumn{1}{c}{\textbf{Acc. (\%)}} \\ \hline \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Multi.-\\Based\end{tabular}}   & AlphaNet                                                   & 320.43             & 0.00               & 320.43           & 1.923               & 65.99             \\
                                                                         & PreNAS-A                                                   & 342.44             & 0.00               & 342.44           & 2.055               & 66.18             \\
                                                                         & PreNAS-B                                                   & 281.17             & 0.00               & 281.17           & 1.687               & 66.03             \\
                                          & PreNAS-C                                                   & 238.64             & 0.00               & 238.64           & 1.432               & 65.89             \\ \hline
                                                                         & DeepShift-MV2                                              & 19.77              & 215.03             & 234.80           & 0.428               & 55.3              \\
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Multi.-\\ Free\end{tabular}} & AdderNet-Res20                                             & 21.23              & 0.00               & 362.45     & 0.373               & 43.7                       \\ \hline
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Multi.-\\ Reduced\end{tabular}} 
& NASA-F-A                                                   & 212.96             & 52.28              & 299.61           & 1.378               & 66.51             \\
                                                                      & NASA-F-B                                                   & 167.59             & 98.40              & 319.25           & 1.186               & 66.18             \\
                                                                         & NASA-F-C                                                   & 159.80             & 93.76              & 306.83           & 1.132               & 65.99             \\
                                                                         & NASA-F-D                                                   & 133.54             & 80.67              & 262.81           & 0.952               & 65.86		\\
									& \rowcolor{dark-green!15} \textbf{Ours-A}                                                                      & \textbf{252.44}    & \textbf{63.96}     & \textbf{350.77}  & \textbf{1.631}      & \textbf{67.24}                           \\
                                                                           & \rowcolor{dark-green!15} \textbf{Ours-B}                               & \textbf{216.02}    & \textbf{54.49}     & \textbf{298.75}  & \textbf{1.395}      & \textbf{66.94}                            \\
                                                                           & \rowcolor{dark-green!15} \textbf{Ours-D}                               & \textbf{169.21}    & \textbf{41.13}     & \textbf{238.76}  & \textbf{1.095}      & \textbf{66.65}              \\ \Xhline{3\arrayrulewidth}             
\end{tabular}} \label{tab:alg-exp-tiny}
\end{table}

==> Tables/hw-cifar10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{1.5pt}
\caption{Comparisons in terms of hardware resource consumption, throughput (\texttt{Thrpt.}), FPS, and accuracy, when tested on CIFAR10.} 
\renewcommand{\arraystretch}{1.2}
\resizebox{\linewidth}{!}{
\begin{threeparttable}{
\begin{tabular}{c||cccc|cc|cccccc}
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c|}{\textbf{Multiplication-Based}}                                      & \multicolumn{2}{c|}{\textbf{Multiplication-Free}}                & \multicolumn{6}{c}{\textbf{Multiplication-Reduced}}                 \\ \cline{2-13} 
                                 & \textbf{AlphaNet}      & \textbf{PreNAS-A}         & \textbf{PreNAS-B}    & \textbf{PreNAS-A-C}        & \textbf{DeepShift-MV2}              & \textbf{AdderNet-MV2}              & \textbf{NASA-F-A} & \textbf{NASA-F-B} & \textbf{NASA-F-C}          & \color{dark-green}\textbf{Ours-A} & \color{dark-green}\textbf{Ours-B} & \color{dark-green}\textbf{Ours-C} \\ \hline \hline
\textbf{Bitwidth}                & \textbf{INT8}          & \textbf{INT8}          & \textbf{INT8}          & \textbf{INT8}          & \textbf{INT8}          & \textbf{INT8}         & \textbf{INT8}               & \textbf{INT8}              & \textbf{INT8}          & \textbf{INT8}            & \textbf{INT8}            & \textbf{INT8}            \\ \hline 
\textbf{\textbf{Strategy}}                & \multicolumn{4}{c|}{\textbf{DSP-Packing}}                                         & \multicolumn{2}{c|}{\textbf{LUT Implementations}} & \multicolumn{6}{c}{\textbf{DSP-Packing + LUT Implementations}}               \\ \hline
\textbf{kLUT}                   & 41.3 (35.32\%)          & 41.6 (35.54\%)            & 41.3 (35.32\%)              & 41.1 (35.11\%)              & 46.2 (39.45\%)                                & 46.7 (39.88\%)                               & 63.9 (54.60\%)              & 80.1 (68.48\%)              & 74.2 (63.00\%)              & 61.7 (52.75\%)            & 65.4 (55.94\%)            & 66.4 (56.73\%)           \\
\textbf{DSP}                     & 545 (43.7\%) & 545 (43.7\%) & 545 (43.7\%) & 545 (43.7\%)  & --                  & --                & 545 (43.7\%) & 545 (43.7\%)   & 545 (43.7\%)   & 545 (43.7\%) & 545 (43.7\%)   & 545 (43.7\%)   \\
\textbf{BRAM}                    & 80 (27.7\%)   & 80 (27.7\%)   & 80 (27.7\%)   & 80 (27.7\%)   & 80 (27.7\%)   & 80 (27.7\%)         & 80 (27.7\%)       & 80 (27.7\%)   & 80 (27.7\%)     & 25.8 (8.9\%)   & 19.4 (6.7\%)   & 19.2 (6.7\%)     \\
\textbf{Freq. (MHz)}              & 200           & 200           & 200           & 200           & 200           & 200          & 200                 & 200               & 200           & 200             & 200             & 200             \\ \hline
\textbf{Latency (ms)}            & 1.08          & 1.27676           & 1.04432           & 0.8872            & 0.66                                & 0.66                               & 0.72              & 0.63              & 0.57              & 0.59            & 0.50            & 0.44   \\
\textbf{Thrpt. (GOPS)}           & 134.9         & 133.9             & 133.8             & 136.1             & 258.4                               & 258.4                              & 228.9             & 308.3             & 310.1             & 315.7           & 336.7           & 357.5  \\
\textbf{GOPS/kLUT}               & 3.265         & 3.219             & 3.237             & 3.313             & 5.598                               & 5.538                              & 3.583             & 3.848             & 4.177             & 5.115           & 5.145           & 5.386  \\
\textbf{GOPS/DSP}                 & 0.248         & 0.246             & 0.245             & 0.250             & --                                  & --                                 & 0.420             & 0.566             & 0.569             & 0.579           & 0.618           & 0.656  \\
\textbf{FPS}                     & 925.9         & 783.2             & 957.6             & 1127.1            & 1515.2                              & 1515.2                             & 1388.9            & 1587.3            & 1754.4            & 1706.2          & 1980.5          & 2273.6 \\ \hline
\textbf{HW Search}           & {\color{dark-green}{\xmark}}     & {\color{dark-green}{\xmark}}              & {\color{dark-green}{\xmark}}                   & {\color{dark-green}{\xmark}}                    & {\color{dark-green}{\xmark}}                    & {\color{dark-green}{\xmark}}                      & {\color{dark-green}{\xmark}}   & {\color{dark-green}{\xmark}}                    &  {\color{dark-green}{\xmark}}            & {\color{purple}{\cmark}}                &{\color{purple}{\cmark}}               & {\color{purple}{\cmark}}                \\
\textbf{Top-1 Acc. (\%)}                 & 95.86         & 96.09             & 95.9              & 95.72             & 91.90                               & 89.50                              & 95.96             & 95.87             & 95.72             & 96.16           & 96.06           & 95.87  \\ \Xhline{3\arrayrulewidth}
\end{tabular}}
\end{threeparttable}} \label{tab:hw-exp-cifar10} 
\end{table*}

==> Tables/hw-cifar100.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{1.5pt}
\caption{Comparisons in terms of hardware resource consumption, throughput (\texttt{Thrpt.}), FPS, and accuracy, when tested on CIFAR10.} 
\renewcommand{\arraystretch}{1.2}
\resizebox{\linewidth}{!}{
\begin{threeparttable}{
\begin{tabular}{c||cccc|cc|cccccc}
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c|}{\textbf{Multiplication-Based}}                                      & \multicolumn{2}{c|}{\textbf{Multiplication-Free}}                & \multicolumn{6}{c}{\textbf{Multiplication-Reduced}}                 \\ \cline{2-13} 
                                 & \textbf{AlphaNet}      & \textbf{PreNAS-A}         & \textbf{PreNAS-B}    & \textbf{PreNAS-A-C}        & \textbf{DeepShift-MV2}              & \textbf{AdderNet-MV2}              & \textbf{NASA-F-A} & \textbf{NASA-F-B} & \textbf{NASA-F-C}          & \color{dark-green}\textbf{Ours-A} & \color{dark-green}\textbf{Ours-B} & \color{dark-green}\textbf{Ours-C} \\ \hline \hline
\textbf{Bitwidth}                & \textbf{INT8}          & \textbf{INT8}          & \textbf{INT8}          & \textbf{INT8}          & \textbf{INT8}          & \textbf{INT8}         & \textbf{INT8}               & \textbf{INT8}              & \textbf{INT8}          & \textbf{INT8}            & \textbf{INT8}            & \textbf{INT8}            \\ \hline 
\textbf{\textbf{Strategy}}                & \multicolumn{4}{c|}{\textbf{DSP-Packing}}                                         & \multicolumn{2}{c|}{\textbf{LUT Implementations}} & \multicolumn{6}{c}{\textbf{DSP-Packing + LUT Implementations}}               \\ \hline
\textbf{kLUT}                   & 41.8 (35.71\%)          & 42.4 (36.22\%)              & 41.8 (35.71\%)              & 41.4 (35.37\%)              & 47.2 (40.31\%)                                & 48.2 (41.16\%)                               & 53.4 (45.63\%)              & 53.8 (45.97\%)              & 58.8 (50.26\%)              & 62.3 (53.21\%)            & 59.5 (50.82\%)            & 59.5 (50.82\%)           \\
\textbf{DSP}                     & 545 (43.7\%) & 545 (43.7\%) & 545 (43.7\%) & 545 (43.7\%)  & --                  & --                & 545 (43.7\%) & 545 (43.7\%)   & 545 (43.7\%)   & 545 (43.7\%) & 545 (43.7\%)   & 545 (43.7\%)   \\
\textbf{BRAM}                    & 80 (27.7\%)   & 80 (27.7\%)   & 80 (27.7\%)   & 80 (27.7\%)   & 80 (27.7\%)   & 80 (27.7\%)         & 80 (27.7\%)       & 80 (27.7\%)   & 80 (27.7\%)     & 39.0 (13.5\%)   & 26.5 (9.2\%)   & 19.2 (6.7\%)     \\
\textbf{Freq. (MHz)}              & 200           & 200           & 200           & 200           & 200           & 200          & 200                 & 200               & 200           & 200             & 200             & 200             \\ \hline
\textbf{Latency (ms)}            & 1.03          & 1.37           & 1.03           & 0.9071            & 0.66                                & 0.66                               & 0.99              & 0.84              & 0.74              & 0.68            & 0.63            & 0.53   \\
\textbf{Thrpt. (GOPS)}           & 147.6         & 138.6             & 147.1             & 143.1             & 258.4                               & 258.4                              & 197.5             & 193.8             & 215.9             & 296.6           & 302.4           & 299.6  \\
\textbf{GOPS/kLUT}               & 3.533         & 3.271             & 3.520             & 3.459             & 5.479                               & 5.366                              & 3.699             & 3.604             & 3.672             & 4.764           & 5.086           & 5.038  \\
\textbf{GOPS/DSP}                 & 0.271         & 0.254             & 0.270             & 0.263             & ---                                 & --                                 & 0.362             & 0.356             & 0.396             & 0.544           & 0.555           & 0.550  \\
\textbf{FPS}                     & 970.9         & 731.0             & 968.8             & 1102.4            & 1515.2                              & 1515.2                             & 1010.1            & 1190.5            & 1351.4            & 1467.5          & 1588.4          & 1880.9 \\ \hline
\textbf{HW Search}           & {\color{dark-green}{\xmark}}     & {\color{dark-green}{\xmark}}              & {\color{dark-green}{\xmark}}                   & {\color{dark-green}{\xmark}}                    & {\color{dark-green}{\xmark}}                    & {\color{dark-green}{\xmark}}                      & {\color{dark-green}{\xmark}}   & {\color{dark-green}{\xmark}}                    &  {\color{dark-green}{\xmark}}            & {\color{purple}{\cmark}}                &{\color{purple}{\cmark}}               & {\color{purple}{\cmark}}                \\
\textbf{Top-1 Acc. (\%)}                & 79.1          & 79.61             & 79.4              & 78.98             & 71.00                               & 63.50                              & 79.68             & 79.42             & 79.17             & 80.09           & 79.85           & 79.63  \\ \Xhline{3\arrayrulewidth}
\end{tabular}}
\end{threeparttable}} \label{tab:hw-exp-cifar10} 
\end{table*}

==> Tables/hw-exp-abl_1.tex <==
\begin{table}[]
\centering
\setlength{\tabcolsep}{6pt}
\caption{Comparisons of search accuracy and search efficiency among various search strategies when tested on Ours-A and CIFAR100} 
\renewcommand{\arraystretch}{1.1}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|c|c|c}
\Xhline{3\arrayrulewidth}
\multicolumn{1}{l|}{\textbf{Coarse Search}} & \multicolumn{1}{l|}{\textbf{Fine Search}} & \multicolumn{1}{l|}{\textbf{Thrpt. (GOPS)}} & \textbf{Time Cost} \\ \hline \hline
{\color{purple}{\xmark}}                                            &  {\color{purple}{\xmark}}                                          &{296.6}                                               &40 minutes                    \\
{\color{dark-green}{\cmark}}                                            & {\color{purple}{\xmark}}                                         &251.6                                            &1 minute                    \\ 
{\color{purple}{\xmark}}                                            & {\color{dark-green}{\cmark}}                                         &289.5                                            &2 minutes                    \\ 
\rowcolor{dark-green!15}  {\color{dark-green}{\cmark}}                                            & {\color{dark-green}{\cmark}}                                         &\textbf{296.6}                                           &\textbf{3 minutes}                    \\ \Xhline{3\arrayrulewidth}
\end{tabular}} \label{table:hw-abl} 
\end{table} 


==> Tables/hw-tiny.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{2.3pt}
\caption{\huihong{Comparisons in terms of hardware resource consumption, throughput (\texttt{Thrpt.}), FPS, and accuracy on Tiny-ImageNet.}} 
\renewcommand{\arraystretch}{1.2}
\resizebox{\linewidth}{!}{
\begin{tabular}{c||cccc|cc|cccccc}
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c|}{\textbf{Multiplication-Based}}                         & \multicolumn{2}{c|}{\textbf{Multiplication-Free}}                                & \multicolumn{6}{c}{\textbf{Multiplication-Reduced}}                   \\ \cline{2-13} 
                                 & \textbf{AlphaNet} & \textbf{PreNAS-A} & \textbf{PreNAS-B} & \multicolumn{1}{c|}{\textbf{PreNAS-C}} & \textbf{AdderNet-ResNet-20}   & \textbf{DeepShift-MV2}  & \textbf{NASA-F-A} & \textbf{NASA-F-B} & \textbf{NASA-F-C} & \color{dark-green}{\textbf{Ours-A}} & \color{dark-green}{\textbf{Ours-B}} & \color{dark-green}{\textbf{Ours-C}}  \\ \hline \hline
\textbf{Bitwidth}                & \textbf{INT8}       & \textbf{INT8}       & \textbf{INT8}       & \textbf{INT8}     & \textbf{INT8}       & \textbf{INT8}   & \textbf{INT8}       & \textbf{INT8}   & \textbf{INT8}   & \textbf{INT8}   & \textbf{INT8}   & \textbf{INT8}   \\ \hline
\textbf{Strategy}                & \multicolumn{4}{c|}{\textbf{DSP-Packing}}                     & \multicolumn{2}{c|}{\textbf{LUT Implementations}}                               & \multicolumn{6}{c}{\textbf{DSP-Packing + LUT Implementations}}        \\ \hline
\textbf{kLUT}                    & 42.9 (36.65\%)          & 43.1 (36.82\%)              & 42.0 (35.88\%)              & 41.7 (35.62\%)              & 48.3 (41.28\%)                                & 60.9 (52.05\%)                               & 52.6 (44.97\%)              & 67.7 (57.89\%)              & 69.2 (59.18\%)              & 54.5 (46.57\%)            & 55.2 (47.17\%)            & 56.3 (48.16\%)            \\
\textbf{DSP}                     & 545 (43.67\%) & 545 (43.67\%)     & 545 (43.67\%)     & 545 (43.67\%)     & --                                  & --                                 & 545 (43.67\%)     & 545 (43.67\%)     & 545 (43.67\%)     & 545 (43.67\%)   & 545 (43.67\%)   & 545 (43.67\%)   \\
\textbf{BRAM}                    & 80 (27.7\%)   & 80 (27.7\%)       & 80 (27.7\%)       & 80 (27.7\%)       & 80 (27.7\%)                         & 80 (27.7\%)                        & 80 (27.7\%)       & 80 (27.7\%)       & 80 (27.7\%)       & 52.5 (18.2\%)     & 44.8 (15.5\%)      & 73.0 (25.3\%)     \\
\textbf{Freq.(MHz)}              & 200           & 200               & 200               & 200               & 200                                 & 200                                & 200               & 200               & 200               & 200             & 200             & 200            \\ \hline
\textbf{Latency (ms)}          & 2.98          & 3.34              & 2.77              & 2.41              & 1.4                                 & 1.04                               & 2                 & 1.65              & 1.27              & 1.68            & 1.42            & 1.11            \\
\textbf{Thrpt. (GOPS)}           & 215.1         & 205.1             & 203.0             & 83.0              & 335.4                               & 368.9                              & 282.4             & 354.7             & 375.6             & 396.7           & 400.1           & 405.6           \\ 
\textbf{GOPS/kLUT}                & 5.015         & 4.760             & 4.836             & 1.991             & 6.945                               & 6.058                              & 5.368             & 5.237             & 5.424             & 7.280           & 7.249           & 7.197          \\
\textbf{GOPS/DSP}                & 0.395         & 0.376             & 0.372             & 0.152             & --                                  & --                                 & 0.518             & 0.651             & 0.689             & 0.728           & 0.734           & 0.744          \\
\textbf{FPS}                     & 335.6         & 299.4             & 361.0             & 414.9             & 714.3                               & 961.5                              & 500.0             & 606.1             & 787.4             & 594.6           & 702.8           & 903.0           \\ \hline
\textbf{Top-1 Acc. (\%)}               & 65.99         & 66.18             & 66.03             & 65.89             & 55.3                                & 43.7                               & 66.51             & 66.18             & 65.86             & 67.24           & 66.94           & 66.65           \\ \Xhline{3\arrayrulewidth}
\end{tabular}} \label{table:hw-exp-tiny} 
\end{table*}



